Spatio-Temporal Trajectory Similarity Measures: A Comprehensive Survey and Quantitative Study

Spatio-temporal trajectory analytics is at the core of smart mobility solutions, which offers unprecedented information for diversified applications such as urban planning, infrastructure development, and vehicular networks. Trajectory similarity measure, which aims to evaluate the distance between two trajectories, is a fundamental functionality of trajectory analytics. In this paper, we propose a comprehensive survey that investigates all the most common and representative spatio-temporal trajectory measures. First, we provide an overview of spatio-temporal trajectory measures in terms of three hierarchical perspectives: Non-learning vs. Learning, Free Space vs. Road Network, and Standalone vs. Distributed. Next, we present an evaluation benchmark by designing five real-world transformation scenarios. Based on this benchmark, extensive experiments are conducted to study the effectiveness, robustness,nefficiency, and scalability of each measure, which offers guidelines for trajectory measure selection among multiple techniques and applications such as trajectory data mining, deep learning, and distributed processing.

==> useless.tex <==
%Sampling Rate in Free Space
\begin{table*}[]
%\vspace{-12mm}
\caption{Robustness of Learning-based Measures vs. Sampling Rate (AIS)}
\small
\vspace{-3mm}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
\makebox[0.13\textwidth][c]{Sample Rate (\%)}                                                                  & \makebox[0.2\textwidth][c]{Measures} & \makebox[0.08\textwidth][c]{DTW}    & \makebox[0.08\textwidth][c]{LCSS}   & \makebox[0.08\textwidth][c]{EDR}    & \makebox[0.08\textwidth][c]{ERP}    & \makebox[0.08\textwidth][c]{Frechet} & \makebox[0.08\textwidth][c]{Hausdorff} \\ \hline
\multirow{2}{*}{$S$=10} & NEUTRAJ                                                        & 0.0087  & 0.0075  & 0.0073 & 0.0082 & 0.0086  & 0.0087                                                \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.2515  & 0.0016  & 0.0078 & 0.0356 & 0.2067  & 0.2520                                                \\ \hline
\multirow{2}{*}{$S$=20} & NEUTRAJ                                                        & 0.0087  & 0.0083  & 0.0087 & 0.0080 & 0.0091  & 0.0091                                                \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.2603 & 0.0019  & 0.0077 & 0.0352 & 0.2151  & 0.2610                                                \\ \hline
\multirow{2}{*}{$S$=40} & NEUTRAJ                                                        & 0.0090  & 0.0080  & 0.0082 & 0.0084 & 0.0086  & 0.0095                                                \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.2590  & 0.00183 & 0.0079 & 0.0351 & 0.2151  & 0.2602                                                \\ \hline
\multirow{2}{*}{$S$=100} & NEUTRAJ                                                        & 0.0082 &0.0094 & 0.0074 &0.0076 &0.0087   &0.0088                                                 \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.25905  &0.0018233 & 0.0079 & 0.0352 &0.2143  & 0.2705                                               \\ \hline
\end{tabular}
\label{tab:SRF}
\vspace{-2mm}
\end{table*}
\begin{table*}[]
%\vspace{-12mm}
\caption{Robustness of Learning-based Measures vs. Sampling Rate (Geolife)}
\small
\vspace{-3mm}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\makebox[0.13\textwidth][c]{Sample Rate (\%)}                                                                  & \makebox[0.2\textwidth][c]{Measures} & \makebox[0.08\textwidth][c]{DTW}    & \makebox[0.08\textwidth][c]{LCSS}   & \makebox[0.08\textwidth][c]{EDR}    & \makebox[0.08\textwidth][c]{ERP}    & \makebox[0.08\textwidth][c]{Frechet} & \makebox[0.08\textwidth][c]{Hausdorff} \\ \hline
\multirow{2}{*}{$S$=10} & NEUTRAJ                                                        & 0.0281 & 0.0217 & 0.0140 & 0.0156 & 0.0178 & 0.0166     \\ \cline{2-8} 
                        & Traj2SimVec                                                     & 0.0106 & 0.3312 & 0.3312 & 0.0271 & 0.0158 & 0.0110 \\ \hline
\multirow{2}{*}{$S$=20} & NEUTRAJ                                                         & 0.0277 & 0.0204 & 0.0113 & 0.0179 & 0.0200 & 0.0183     \\ \cline{2-8} 
                        & Traj2SimVec                                                   & 0.0094 & 1.000 & 1.000 & 0.0245 & 0.0158 & 0.0110 \\ \hline
\multirow{2}{*}{$S$=40} & NEUTRAJ                                                         &0.0277 & 0.0206 & 0.0121 & 0.0210 & 0.0220 & 0.0214    \\ \cline{2-8} 
                        & Traj2SimVec                                                   & 0.0094 & 1.000 & 1.000 & 0.0245 & 0.0158 & 0.0112  \\ \hline
\multirow{2}{*}{$S$=100} & NEUTRAJ & 0.0277 & 0.0212 & 0.0204 & 0.0252 & 0.0258 & 0.0249
                                            \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.0366 & 1.000 & 1.000 & 0.0215 & 0.0131 & 0.0513                                    \\ \hline
\end{tabular}
\label{tab:SRFG}
\vspace{-2mm}
\end{table*}

%Noise in Free Space
\begin{table*}[]
\caption{Robustness of Learning-based Measures vs. Noise Ratio (AIS)}
\vspace{-3mm}
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\makebox[0.13\textwidth][c]{Noise Ratio (\%)}                                                                  & \makebox[0.2\textwidth][c]{Measures} & \makebox[0.08\textwidth][c]{DTW}    & \makebox[0.08\textwidth][c]{LCSS}   & \makebox[0.08\textwidth][c]{EDR}    & \makebox[0.08\textwidth][c]{ERP}    & \makebox[0.08\textwidth][c]{Frechet} & \makebox[0.08\textwidth][c]{Hausdorff} \\ \hline
\multirow{1.2}{*}{$N$=0} & NEUTRAJ                                                        & 0.0082 &0.0094 & 0.0074 &0.0076 &0.0087   &0.0088                                                 \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.25905  &0.0018233 & 0.0079 & 0.0352 &0.2143  & 0.2705                                               \\ \hline
\multirow{1.2}{*}{$N$=13} & NEUTRAJ                                                        & 0.0091 & 0.0080 & 0.0073 & 0.0079 & 0.0087  & 0.0085    \\ \cline{2-8} 
                                                                      & Traj2SimVec                                                    & 0.2460 & 0.0017 & 0.0079 & 0.0345 & 0.2091  & 0.2583    \\ \hline
\multirow{1.2}{*}{$N$=16} & NEUTRAJ                                                        & 0.0092 & 0.0071 & 0.0080 & 0.0082 & 0.0091  & 0.0085    \\ \cline{2-8} 
                                                                      & Traj2SimVec                                                    & 0.2464 & 0.0021 & 0.0080 & 0.0348 & 0.2053  & 0.2558    \\ \hline
\multirow{1.2}{*}{$N$=19} & NEUTRAJ                                                        & 0.0083 & 0.0071 & 0.0066 & 0.0081 & 0.0087  & 0.0084    \\ \cline{2-8} 
                                                                      & Traj2SimVec                                                    & 0.2403 & 0.0017 & 0.0078 & 0.0334 & 0.2034  & 0.2540    \\ \hline
\end{tabular}
\label{tab:NF}
\vspace{-2mm}
\end{table*}
\begin{table*}[]
\caption{Robustness of Learning-based Measures vs. Noise Ratio (Geolife)}
\vspace{-3mm}
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\makebox[0.13\textwidth][c]{Noise (\%)}                                                                  & \makebox[0.2\textwidth][c]{Measures} & \makebox[0.08\textwidth][c]{DTW}    & \makebox[0.08\textwidth][c]{LCSS}   & \makebox[0.08\textwidth][c]{EDR}    & \makebox[0.08\textwidth][c]{ERP}    & \makebox[0.08\textwidth][c]{Frechet} & \makebox[0.08\textwidth][c]{Hausdorff} \\ \hline
\multirow{1.2}{*}{$N$=0} & NEUTRAJ & 0.0277 & 0.0212 & 0.0204 & 0.0252 & 0.0258 & 0.0249
                                            \\ \cline{2-8} 
                        & Traj2SimVec                                                    & 0.0366 & 1.000 & 1.000 & 0.0215 & 0.0131 & 0.0513                                    \\ \hline
\multirow{1.2}{*}{$N$=13} & NEUTRAJ                                                     & 0.0276 & 0.0223 & 0.0203 & 0.0243 & 0.0247 & 0.0227 \\ \cline{2-8} 
                         & Traj2SimVec                                                  & 0.0094 & 1.000 & 1.000 & 0.0255 & 0.0158 & 0.0110                                    \\ \hline
\multirow{1.2}{*}{$N$=16} & NEUTRAJ                                                     & 0.0259 & 0.0201 & 0.0107 & 0.0283 & 0.0259 & 0.0251         \\ \cline{2-8} 
                            & Traj2SimVec                                               & 0.0094 & 1.000 & 1.000 & 0.0249 & 0.0158 & 0.0110                                 \\ \hline
\multirow{1.2}{*}{$N$=19} & NEUTRAJ                                                     & 0.0262 & 0.0200 & 0.0103 & 0.0266 & 0.0259 & 0.0254          \\ \cline{2-8} 
                          & Traj2SimVec                                                 & 0.0094 & 1.000 & 1.000 & 0.0252 & 0.0158 & 0.0110                                    \\ \hline
\end{tabular}
\label{tab:NFG}
\vspace{-2mm}
\end{table*}

%Efficiency
\begin{table}[]
\caption{Efficiency of Learning-based Measures in Free Space (AIS)}
\vspace{-3mm}
\small
\begin{tabular}{|c|cc|cc|}
\hline
        & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{NEUTRAJ}}          & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{Traj2SimVec}}      \\ \cline{2-5} %\hline
\multirow{-2}{*}{\makebox[0.09\textwidth][c]{Measures}}          & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} \\ \hline
DTW       & \multicolumn{1}{c|}{125.01}   & 46.80 & \multicolumn{1}{c|}{135.19}   & 6.59 \\ \hline
LCSS      & \multicolumn{1}{c|}{107.87}   & 42.59 & \multicolumn{1}{c|}{143.94}   & 5.97 \\ \hline
EDR       & \multicolumn{1}{c|}{126.02}   & 45.89  & \multicolumn{1}{c|}{138.36}   & 6.13 \\ \hline
ERP       & \multicolumn{1}{c|}{111.30}    & 47.14 & \multicolumn{1}{c|}{141.94}   & 5.99 \\ \hline
Frechet   & \multicolumn{1}{c|}{104.01}   & 42.80 & \multicolumn{1}{c|}{136.37}   & 7.46 \\ \hline
Hausdorff & \multicolumn{1}{c|}{113.38}   & 46.89  & \multicolumn{1}{c|}{135.45}   & 6.61  \\ \hline
\end{tabular}
\label{tab:efficiencyF}
\vspace{-4mm}
\end{table}
\begin{table}[]
\caption{Efficiency of Learning-based Measures in Free Space (Geolife)}
\vspace{-3mm}
\small
\begin{tabular}{|c|cc|cc|}
\hline
        & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{NEUTRAJ}}          & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{Traj2SimVec}}      \\ \cline{2-5} %\hline
\multirow{-2}{*}{\makebox[0.09\textwidth][c]{Measures}}          & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} \\ \hline
DTW       & \multicolumn{1}{c|}{58.72}	   & 9.70 & \multicolumn{1}{c|}{66.95}   & 2.96 \\ \hline
LCSS      & \multicolumn{1}{c|}{59.25}   & 9.64 & \multicolumn{1}{c|}{65.83}   & 3.36 \\ \hline
EDR       & \multicolumn{1}{c|}{54.16}   & 9.01  & \multicolumn{1}{c|}{66.58}   & 3.35 \\ \hline
ERP       & \multicolumn{1}{c|}{57.64}    & 9.43 & \multicolumn{1}{c|}{65.85}   & 3.94 \\ \hline
Frechet   & \multicolumn{1}{c|}{53.20}   & 9.61 & \multicolumn{1}{c|}{66.55}   & 3.65 \\ \hline
Hausdorff & \multicolumn{1}{c|}{57.80}   & 9.60  & \multicolumn{1}{c|}{63.30}   & 3.59  \\ \hline
\end{tabular}
\label{tab:efficiencyFG}
\vspace{-4mm}
\end{table}
\begin{table}[]
\caption{Efficiency of Learning-based Measures in Road Network (T-Drive)}
\vspace{-3mm}
\small
\begin{tabular}{|c|cc|cc|}
\hline
        & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{GTS}}                      & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{ST2Vec}}                   \\ \cline{2-5}%\hline
\multirow{-2}{*}{\makebox[0.09\textwidth][c]{Measures}}        & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} \\ \hline
NetLCSS & \multicolumn{1}{c|}{8.62}         & 2.67       & \multicolumn{1}{c|}{171.84}       & 3.61     \\ \hline
NetDTW  & \multicolumn{1}{c|}{8.66}         & 2.66      & \multicolumn{1}{c|}{166.04}       & 2.56      \\ \hline
TP      & \multicolumn{1}{c|}{8.64}         & 2.63      & \multicolumn{1}{c|}{165.75}       & 3.14      \\ \hline
NetERP  & \multicolumn{1}{c|}{9.83}         & 2.82     & \multicolumn{1}{c|}{212.68}       & 12.32     \\ \hline
\end{tabular}
\label{tab:efficiencyR}
\vspace{-2mm}
\end{table}
\begin{table}[]
\caption{Efficiency of Learning-based Measures in Road Network (Porto)}
\vspace{-3mm}
\small
\begin{tabular}{|c|cc|cc|}
\hline
        & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{GTS}}                      & \multicolumn{2}{c|}{\makebox[0.16\textwidth][c]{ST2Vec}}                   \\ \cline{2-5}%\hline
\multirow{-2}{*}{\makebox[0.09\textwidth][c]{Measures}}        & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} & \multicolumn{1}{c|}{\makebox[0.07\textwidth][c]{$T_{tra}$(s)}} & \multicolumn{1}{c|}{$Q$(ms)} \\ \hline
NetLCSS & \multicolumn{1}{c|}{6.31}         & 0.96       & \multicolumn{1}{c|}{106.22}       & 1.23     \\ \hline
NetDTW  & \multicolumn{1}{c|}{6.41}         & 1.33      & \multicolumn{1}{c|}{106.80}       & 1.20      \\ \hline
TP      & \multicolumn{1}{c|}{6.35}         & 1.08      & \multicolumn{1}{c|}{119.15}       & 1.15      \\ \hline
NetERP  & \multicolumn{1}{c|}{6.34}         & 0.97     & \multicolumn{1}{c|}{126.29}       & 1.20     \\ \hline
\end{tabular}
\label{tab:efficiencyRP}
\vspace{-4mm}
\end{table}
